The Transactional Conflict Problem

The transactional conflict problem arises in transactional systems whenever two or more concurrent transactions clash on a data item. While the standard solution to such conflicts is to immediately abort one of the transactions, some practical systems consider the alternative of delaying conflict resolution for a short interval, which may allow one of the transactions to commit. The challenge in the transactional conflict problem is to choose the optimal length of this delay interval so as to minimize the overall running time penalty for the conflicting transactions. In this paper, we propose a family of optimal online algorithms for the transactional conflict problem. Specifically, we consider variants of this problem which arise in different implementations of transactional systems, namely "requestor wins" and "requestor aborts" implementations: in the former, the recipient of a coherence request is aborted, whereas in the latter, it is the requestor which has to abort. Both strategies are implemented by real systems. We show that the requestor aborts case can be reduced to a classic instance of the ski rental problem, while the requestor wins case leads to a new version of this classical problem, for which we derive optimal deterministic and randomized algorithms. Moreover, we prove that, under a simplified adversarial model, our algorithms are constant-competitive with the offline optimum in terms of throughput. We validate our algorithmic results empirically through a hardware simulation of hardware transactional memory (HTM), showing that our algorithms can lead to non-trivial performance improvements for classic concurrent data structures.

==> requestor_aborts.tex <==
\section{Requestor Aborts General}
	\noindent In the requestor aborts case we have the following cost function 
	
	\begin{align}
		\text{Cost(p(x),y)} = \int_{0}^{y} ( k - 1 )( x + B ) p(x) dx + ( k - 1 ) \int_{y}^{\frac{B}{k-1}} y p(x) dx		
	\end{align}
	
	Thus our Lagrangian function looks as follows
	
	\begin{align*}
	L(p(x),\lambda_1, \lambda_2) = &\int_{0}^{\frac{B}{k-1}} \left( \frac{\text{Cost(p(x),y)}}{(k-1)y}  -\lambda_1 - \lambda_2 y \right)\pi(y) dy \\
	&+ \pi(k) \cdot \left( \int_{0}^{\frac{B}{k-1}} \frac{( k - 1 ) ( x + B )}{B} p(x) dx - \lambda_1 - \lambda_2l \right) \\
	& + \lambda_1 + \lambda_2 \mu
	\end{align*}
	
	To get a meaningful result we introduce the following two constraints
	
	\begin{align}
	\frac{\text{Cost(p(x),y)}}{(k-1)y} &= \lambda_1 + \lambda_2 y \label{constr_1} \\
	\int_{0}^{\frac{B}{k-1}} \frac{( k - 1 ) ( x + B )}{B} p(x) dx &= \lambda_1 + \lambda_2l \label{constr_2}
	\end{align}
	
	By differentiating the first constraint twice w.r.t. $y$ we get
	
	\begin{align*}
	\left[ \int_{0}^{y}( k - 1 ) ( x + B ) p(x) dx + ( k - 1)  \int_{y}^{\frac{B}{k-1}} y p(x) dx\right]'' &= \left[( k-1 ) y ( \lambda_1 + \lambda_2 y) \right]'' \\
	\left[ \int_{0}^{y} ( x + B ) p(x) dx + \int_{y}^{\frac{B}{k-1}} y p(x) dx\right]'' &= \left[y ( \lambda_1 + \lambda_2 y) \right]'' \\
	\left[ P(y) ( y + B ) - P(0) B  - \int_{0}^{y} P(x) dx +  y \left( P(\frac{B}{k-1}) - P(y)\right)\right]'' &= 2 \lambda_2 \\
	\left[ P(y) B  - P(0) B  - \mathcal{P}(y) + \mathcal{P}(0) + y  P(\frac{B}{k-1})\right]'' &= 2 \lambda_2 \\
	\left[ p(y) B - P(y) + P(\frac{B}{k-1})\right]' &= 2 \lambda_2 \\
	p'(y) B -  p(y)&= 2 \lambda_2 \\
	%	p'(y) &= \frac{2 (j-1) \lambda_2 + ( j-2 ) p(y)}{y + B}
	\end{align*}
	
	Solving this first order differential equation gives us
	
	\begin{align}
		p(y) = \alpha e^{\frac{y}{B}} - 2 \lambda_2 \label{strategy}
	\end{align}
	
	We can solve for $\alpha$ by using the fact that $p(y)$ is a PDF
	
	\begin{align}
		\alpha = \frac{( k - 1 ) + 2 B \lambda_2}{B ( e^{\frac{1}{k-1}} -1) ( k - 1 )} \label{alpha}
	\end{align}
	
	By substituting \ref{strategy} into our constraint \ref{constr_1} we get
	
	\begin{align*}
		( \alpha B e^{\frac{y}{B}} - 2 \lambda_2 y ) B - \alpha B^2 - \alpha B^2 e^{\frac{y}{B}} +  \lambda_2 y^2 + \alpha B^2 + y \alpha B e^{\frac{1}{k-1}} - 2 y \lambda_2 \frac{B}{k-1} &= y ( \lambda_1 + \lambda_2 y) \\
		\alpha ( -B^2 + B^2 + B^2e^{\frac{y}{B}} - B^2e^{\frac{y}{B}} + y B e^{\frac{1}{k-1}} ) - \lambda_2 ( 2 y B - y^2 + 2 y \frac{B}{k-1} ) &= y ( \lambda_1 + \lambda_2 y) \\
		\alpha B e^{\frac{1}{k-1}} - \lambda_2 ( 2 B + 2 \frac{B}{k-1}) &= \lambda_1
	\end{align*}
	
	Using \ref{alpha} we get
	
	\begin{align}
		\frac{e^{\frac{1}{k-1}}}{e^{\frac{1}{k-1}} - 1} - \lambda_2 \cdot 2 \left ( B - \frac{B}{ ( e^{\frac{1}{k-1}} - 1 ) ( k - 1 )} \right)&= \lambda_1 \label{constr1_solved}
	\end{align}
	
	Similarly substituting \ref{strategy} into constraint \ref{constr_2} we get
	
	\begin{align}
		\alpha B e^{\frac{1}{k-1}} - \lambda_2 \left( 2 B + \frac{B}{k-1} \right) &= \lambda_1 + \lambda_2 l  \nonumber \\
		\frac{e^{\frac{1}{k-1}}}{e^{\frac{1}{k-1}} - 1} - \lambda_2 \cdot 2 \left ( \frac{B}{2 ( k - 1 )} + B + \frac{l}{2}  - \frac{B e^{\frac{1}{k-1}}}{ ( e^{\frac{1}{k-1}} - 1 ) ( k - 1 )}\right) &= \lambda_1 \label{constr2_solved}
	\end{align}
	
	In order for \ref{constr1_solved} and \ref{constr2_solved} to be true at the same time we need
	
	\begin{align}
		l &= \frac{B}{k-1} \label{constr_l}
	\end{align}
	
	Since we know that $p(y)$ is a PDF we know that $\forall y \in [0, \frac{B}{k-1}].p(y) \geq 0$ and thus we get
	
	\begin{align*}
		\left(1 - \frac{e^{\frac{y}{B}}}{( e^{\frac{1}{k-1}} - 1 ) ( k - 1 )} \right)\lambda_2 &\leq \frac{e^{\frac{y}{B}}}{2 B ( e^{\frac{1}{k-1}} - 1 )}
	\end{align*}
	
	We further know that $\forall y \in [0, \frac{B}{k-1}].p(y) \leq 1$ and thus we get the following constraints on $\lambda_2$
	
	\begin{align}
		\lambda_2 &\leq \frac{ ( k - 1 ) e^{\frac{y}{B}}}{2 B (( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - e^{\frac{y}{B}})}, \text{  if } 0 \leq y \leq B \log{\left(( k - 1 ) (e^{\frac{1}{k-1}} - 1 )\right)} \label{lambda2_1}\\
		\lambda_2 &> \frac{ ( k - 1 ) e^{\frac{y}{B}}}{2 B (( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - e^{\frac{y}{B}})}, \text{  if } B \log{\left(( k - 1 ) (e^{\frac{1}{k-1}} - 1 )\right)} < y \leq \frac{B}{k-1} \label{lambda2_2}
	\end{align}
	
	We immediately realize that the r.h.s. of \ref{lambda2_1} is positive and strictly increasing, whereas the r.h.s. of \ref{lambda2_2} is negative. Thus we now know that we must have
	
	\begin{align*}
		0 \leq \lambda_2 \leq \frac{k-1}{2 B (( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)}
	\end{align*}
	
	Thus our problem becomes
	
	\begin{align}
		\max_{\lambda_1, \lambda_2} \lambda_1 + \lambda_2\mu \text{ s.t. } \nonumber \\
		\frac{e^{\frac{1}{k-1}}}{e^{\frac{1}{k-1}} - 1} - \lambda_2 \cdot 2 \left ( B - \frac{B e^{\frac{1}{k-1}}}{ ( e^{\frac{1}{k-1}} - 1 ) ( k - 1 )} + B \right)&= \lambda_1 \\
		\frac{e^{\frac{1}{k-1}}}{e^{\frac{1}{k-1}} - 1} - \lambda_2 \cdot 2 \left ( \frac{B}{2 ( k - 1 )} + B + \frac{l}{2}  - \frac{B e^{\frac{1}{k-1}}}{ ( e^{\frac{1}{k-1}} - 1 ) ( k - 1 )}\right) &= \lambda_1 \\
		\forall \lambda_1  \geq 0, 0 \leq \lambda_2 \leq \frac{k-1}{2 B (( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)} \text{ and } y \in [0,B] \nonumber
	\end{align}
	
	We already realized that \ref{constr_l}. We further remind ourselves that the solutions to this linear program have to form a convex polytope and that each basic feasible solution is a corner point of that polytope. Therefore we get the following two corner points
	
	\begin{align*}
		c_1 = \left(\frac{e^{\frac{1}{k-1}}}{e^{\frac{1}{k-1}} - 1},0\right) \text{ and } c_2 = \left(1,\frac{k - 1 }{2 B (( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)}\right)
	\end{align*}
	
	This gives us the following $C$'s
	
	\begin{align*}
		C_1 = \frac{e^{\frac{1}{k-1}}}{e^{\frac{1}{k-1}} - 1} \text{ and } C_2 = 1 + \frac{\mu ( k - 1 )}{2 B (( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)}
	\end{align*}
	
	Notice that for $\lambda_2 = 0$ we do not take the mean into account and thus are left with the solution for the non-constrained ski rental problem. For $\lambda_2 \neq 0$ we realize that $C_2 < C_1$ is only valid for small values of $\mu$. More precisely, $C_2 < C_1, \text{ for }  \frac{\mu + 2(( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)}{B} < 2(( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)$. For $B > 1$ it simplifies to $\frac{\mu}{B-1} < 2(( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)$. Thus we have finally found our two optimal strategies, namely
	\begin{align*}
	p(x) = \begin{cases}
	\frac{( k - 1 )}{B (( e^{\frac{1}{k-1}} - 1 ) ( k - 1 ) - 1)} ( e^{\frac{y}{B}} - 1 ), &0 \leq x \leq \frac{B}{k-1} \\
	0, &\text{else}
	\end{cases}, \text{ if } \frac{\mu + 2(( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1)}{B} < 2(( k - 1 ) (e^{\frac{1}{k-1}} - 1 ) - 1) \\
	\end{align*}
	and
	\begin{align*}
	p(x) = \begin{cases}
	\frac{( k - 1 )}{B ( e^{\frac{1}{k-1}} -1) ( k - 1 )} e^{\frac{y}{B}}, &0 \leq x \leq \frac{B}{k-1} \\
	0, &\text{else}
	\end{cases}, \text{ else } 
	\end{align*}

	
	\newpage
	
	Useful results:
	
	\begin{align*}
		\int p(y) dy &= \alpha B e^{\frac{y}{B}} - 2 \lambda_2 y \\
		\int \int p(y) dy &= \alpha B^2 e^{\frac{y}{B}} -  \lambda_2 y^2 \\
	\end{align*}
	
	


==> requestor_wins.tex <==




\section{Requestor Wins General}
\begin{align*}
	\text{Cost}(p(x),y) &= \int_{0}^{y}(kx + B) p(x) dx + (k-1) \int_{y}^{\frac{B}{k-1}} y p(x) dx
\end{align*}
the  Lagrangian function looks as follows
\begin{align*}
	L(p(x),\lambda_1, \lambda_2) = &\int_{0}^{\frac{B}{k-1}} \left( \frac{\text{Cost(p(x),y)}}{(k-1)y}  -\lambda_1 - \lambda_2 y \right)\pi(y) dy \\
	&+ \pi(k) \cdot \left( \int_{0}^{\frac{B}{k-1}} \frac{kx+B}{B} p(x) dx - \lambda_1 - \lambda_2k \right) \\
	& + \lambda_1 + \lambda_2 \mu
\end{align*}

To get a meaningful result we introduce the following two constraints

\begin{align*}
	\frac{\text{Cost(p(x),y)}}{(k-1)y} &= \lambda_1 + \lambda_2 y \\
	\int_{0}^{\frac{B}{k-1}} \frac{kx+B}{B} p(x) dx &= \lambda_1 + \lambda_2K 
\end{align*}

By differentiating the first constraint twice w.r.t. $y$ we get

\begin{align*}
	\left[ \int_{0}^{y}(kx + B) p(x) dx + (k-1) \int_{y}^{\frac{B}{k-1}} y p(x) dx\right]'' &= \left[( k-1 ) y ( \lambda_1 + \lambda_2 y) \right]'' \\
	\left[ P(y) ( ky + B ) - P(0) B  - \int_{0}^{y} k P(x) dx +  (k-1) y \left( P(\frac{B}{k-1}) - P(y)\right)\right]'' &= 2 (k-1) \lambda_2 \\
	\left[ P(y) ( y + B ) - P(0) B  - k \mathcal{P}(y) + k \mathcal{P}(0) + (k-1) y  P(\frac{B}{k-1})\right]'' &= 2 (k-1) \lambda_2 \\
	\left[ p(y) ( y + B ) + P(y)  - k P(y) + (k-1) P(\frac{B}{k-1})\right]' &= 2 (k-1) \lambda_2 \\
	p'(y) ( y + B ) - ( k-2 ) p(y)&= 2 (k-1) \lambda_2 \\
%	p'(y) &= \frac{2 (j-1) \lambda_2 + ( j-2 ) p(y)}{y + B}
\end{align*}

by solving this first order differential equation we get

\begin{align*}
	p(y) &= \alpha ( B+y )^{ k-2 } - \frac{2\lambda_2 ( k - 1 )}{k-2}
\end{align*}

Using the fact that $p(x)$ is a PDF we can solve for $\alpha$

\begin{align*}
	\alpha &= \frac{B ( k - 1 ) k ( 2 \lambda_2 B+ k - 2 )}{( k - 2 ) \left[ ( k - 1 ) ( \frac{ B k }{ k - 1 })^k - k B^k \right]} \\
	&= \frac{\lambda_2 ( 2 B^2 k ( k - 1 ))}{ (k - 2 ) \left[ ( k - 1 ) ( \frac{ B k }{ k - 1 })^k - k B^k \right]} + \frac{B ( k - 1 ) k}{  ( k - 1 ) ( \frac{ B k }{ k - 1 })^k - k B^k } \\
\end{align*}

Note:

\begin{align*}
	P(y) &= \frac{\alpha ( B + y )^{ k-1 }}{k-1} - \lambda_2 \frac{2 ( k-1) y}{k-2} \\
	\mathcal{P}(y) &= \frac{\alpha (B+y)^k}{k ( k-1 )} - \lambda_2 \frac{(k-1) y^2}{k-2}
\end{align*}

Substituting $p(y)$ into our first constraint yields

\begin{align*}
	-k \left[ \mathcal{P}(y) - \mathcal{P}(0) \right] + P(y) ( y + B ) - P(0) B + ( k - 1 ) y P\left(\frac{B}{k-1}\right) = ( k - 1 ) y (\lambda_1 + \lambda_2 y ) \\
	-\lambda_2 \frac{2 B}{k - 2} +  P\left(\frac{B}{k-1}\right) &= \lambda_1\\
	-2\lambda_2 \frac{2 B}{k - 2}+\alpha \frac{\left( \frac{Bk}{k-1} \right)^k}{Bk} &= \lambda_1 \\
	\lambda_2 \left(\frac{2B^2k \left( \frac{Bk}{k-1} \right)^{k-1}}{( k - 2 ) \left[ ( k - 1 ) ( \frac{ B k }{ k - 1 })^k - k B^k \right]}-\frac{4B}{k-2}\right) +  \frac{Bk \left( \frac{Bk}{k-1} \right)^{k-1}}{\left[ ( k - 1 ) ( \frac{ B k }{ k - 1 })^k - k B^k \right]}  &= \lambda_1  \\
\lambda_2 \left( \frac{2B}{k-2} \cdot \frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}}-\frac{4B}{k-2} \right)+\frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}} &= \lambda_1
\\
\end{align*}

$p(x)$ is a PDF so we have $p(x) \ge 0$ for $x \in [0, \frac{B}{k-1}]$, this means that $P(x) = \alpha ( B + x )^{ k-2 }- 
\frac{2\lambda_2(k-1)}{k-2} \ge 0$. $\alpha > 0$ and $B>0$, so it is enough to check if $P(0) \ge 0$. This gives us following constraint on $\lambda_2$:

\begin{align*}
\alpha B^{ k-2} 
 & \ge \frac{2\lambda_2(k-1)}{k-2} \\
 \frac{2\lambda_2k(k-1)}{(k-2)\left(\frac{k^{k-1}}{(k-1)^{k-1}}-1\right)}+\frac{k-1}{B\left(\frac{k^{k-1}}{(k-1)^{k-1}}-1\right)} &\ge \frac{2\lambda_2(k-1)}{k-2}\\
 \frac{2\lambda_2}{k-2}\left(1-\frac{(k-1)^{k-1}}{k^{k-1}-(k-1)^{k-1}} \right) &\le \frac{(k-1)^{k-1}}{B\left(k^{k-1}-(k-1)^{k-1}\right)}\\
 \lambda_2 \le \frac{2(k-2)}{B}\frac{\frac{(k-1)^{k-1}}{k^{k-1}-(k-1)^{k-1}}}{1-\frac{(k-1)^{k-1}}{k^{k-1}-(k-1)^{k-1}}} &= \frac{2(k-2)(k-1)^{k-1}}{B\left(k^{k-1}-2(k-1)^{k-1}\right)}
 \end{align*}
 
 this gives us the following constraints:
\begin{align*} 
 \lambda_2 \left( \frac{2B}{k-2} \cdot \frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}}-\frac{4B}{k-2} \right)+\frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}} &= \lambda_1 \\
  \lambda_2 \left( \frac{2B}{k-2} \cdot \frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}}-\frac{4B}{k-2} + \frac{B}{k-1}-K \right)+\frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}} &= \lambda_1\\
0\le  \lambda_2  \le \frac{2(k-2)(k-1)^{k-1}}{B\left(k^{k-1}-2(k-1)^{k-1}\right)}
 \end{align*}
 It is easy to see that we must have $K=\frac{B}{k-1}$.
 We also know the solutions of LP form a convex polytope and this gives us two corner points : 
$\left(\frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}}, 0\right)$ and
$\left(\frac{k^{k-1}-2(k-1)^{k-1}}{k^{k-1}-(k-1)^{k-1}}, \frac{2(k-2)(k-1)^{k-1}}{B\left(k^{k-1}-2(k-1)^{k-1}\right)}\right)$.  The corresponding ratios are : $\frac{k^{k-1}}{k^{k-1}-(k-1)^{k-1}}$ and $\frac{k^{k-1}-2(k-1)^{k-1}}{k^{k-1}-(k-1)^{k-1}}+\frac{2\mu(k-2)(k-1)^{k-1}}{B\left(k^{k-1}-2(k-1)^{k-1}\right)}$. 
We get that if $\frac{\mu}{B} \le \frac{k^{k-1}-2(k-1)^{k-1}}{(k-2)\left(k^{k-1}-(k-1)^{k-1}\right)}$ the optimal PDF is :
$$
P(x)=
\begin{cases}
\frac{(B+x)^{k-2}(k-1)^k\left( 2(k-1)^{k-1}+k^{k-1}\right)}{B^{k-1}\left(k^{k-1}-(k-1)^{k-1}\right)\left(k^{k-1}-2(k-1)^{k-1}\right)}-\frac{4(k-1)^k}{B\left(k^{k-1}-2(k-1)^{k-1}\right)}, & \text{if } 0\le x \le \frac{B}{k-1}\\
0, & \text{otherwise}\\
\end{cases}
$$
and otherwise the optimal  PDF is :
$$
P(x)=
\begin{cases}
\frac{(B+x)^{k-2}(k-1)^k}{B^{k-1}\left(k^{k-1}-(k-1)^{k-1}\right)} , & \text{if } 0\le x \le \frac{B}{k-1}\\
0, & \text{otherwise}\\
\end{cases}
$$

